Non Holonomic Collision Avoidance of Dynamic Obstacles under Non-Parametric Uncertainty: A Hilbert Space Approach

We consider the problem of an agent/robot with non-holonomic kinematics avoiding many dynamic obstacles. State and velocity noise of both the robot and obstacles as well as the robot's control noise are modelled as non-parametric distributions as often the Gaussian assumptions of noise models are violated in real-world scenarios. Under these assumptions, we formulate a robust MPC that samples robotic controls effectively in a manner that aligns the robot to the goal state while avoiding obstacles under the duress of such non-parametric noise. In particular, the MPC incorporates a distribution matching cost that effectively aligns the distribution of the current collision cone to a certain desired distribution whose samples are collision-free. This cost is posed as a distance function in the Hilbert Space, whose minimization typically results in the collision cone samples becoming collision-free. We compare and show tangible performance gain with methods that model the collision cone distribution by linearizing the Gaussian approximations of the original non-parametric state and obstacle distributions. We also show superior performance with methods that pose a chance constraint formulation of the Gaussian approximations of non-parametric noise without subjecting such approximations to further linearizations. The performance gain is shown both in terms of trajectory length and control costs that vindicates the efficacy of the proposed method. To the best of our knowledge, this is the first presentation of non-holonomic collision avoidance of moving obstacles in the presence of non-parametric state, velocity and actuator noise models.

==> chapters/simulations-and-validation.tex <==
\section{Simulations and Validation}
This section presents various simulated examples of navigation of a quadcopter amongst dynamic obstacles in the XY plane. For this, we are approximating the motion model of our quadcopter as a double integrator system.
The inputs represent the change in linear and angular velocities subject to non-gaussian uncertainity. We are also subjecting the positions and velocities of the obstacles and the agent to similar perturbations. The error distributions are depicted in fig

1) Comparison of RKHS based approach with Linear and Non Linear model of PVO for Single Obstacle:\\
i) RKHS based algorithm: The results for this case  are summarized in fig  below. In case of RKHS, the first step to get the solution is the construction of the desired distribution. Then, we need to select the degree of the polynomial kernel used. Subsequently, we need to select an appropriate control which makes our current distribution as close as possible to the desired distribution. This is done by select a control for Which the distance between u1 and u2 is least. It is evident that with increase in value of d, the degree overlapping between the desired distribution and our current distribution increases. This results in less collision between the samples of the agent and the obstacle as evident in fig. This also results in more navigation time with increase in value of d.\\
ii) Linearized Probabilistic Velocity Obstacle: In case of Linearized PVO, the surrogate constraints given by equation  are used. These constraints along with the cost function given by () are used to model an optimization problem. Thus, the change in linear and angular velocities are calculated.  The number of collisions was found out to be almost zero which was much lower than the expected value of .This can be attributed to the error in approximation of the collision cone as seen in fig. This lead to over-estimation of the number of collisions which resulted in a much more conservative path.


